Character Matters: Video Story Understanding with Character-Aware Relations

Different from short videos and GIFs, video stories contain clear plots and lists of principal characters. Without identifying the connection between appearing people and character names, a model is not able to obtain a genuine understanding of the plots. Video Story Question Answering (VSQA) offers an effective way to benchmark higher-level comprehension abilities of a model. However, current VSQA methods merely extract generic visual features from a scene. With such an approach, they remain prone to learning just superficial correlations. In order to attain a genuine understanding of who did what to whom, we propose a novel model that continuously refines character-aware relations. This model specifically considers the characters in a video story, as well as the relations connecting different characters and objects. Based on these signals, our framework enables weakly-supervised face naming through multi-instance co-occurrence matching and supports high-level reasoning utilizing Transformer structures. We train and test our model on the six diverse TV shows in the TVQA dataset, which is by far the largest and only publicly available dataset for VSQA. We validate our proposed approach over TVQA dataset through extensive ablation study.

==> algorithm/naming.tex <==
\begin{algorithm}
    \caption{Character Face Naming}
    \begin{algorithmic}[1]
        \REQUIRE Subtitles $S = \{S_i\}$, feature vectors $V = \{V_j\}$ for all faces $F = \{F_j\}$, the principal character list $M$ for the TV show.
        \STATE Let $k$ = the length of $M$ + 1, the additional 1 is for background characters.
        \STATE Utilize $k$-means to cluster the face features $V$ into $k$ groups. Each $V_j$ is assigned a group number label $L_j$, where $L_j \in \{0, 1, ..., k-1\}$.
        \STATE Let $\mathcal{C}$ be a zero co-occurrence matrix between $k$ groups and all principal characters in $M$.
        \FOR {every $S_i$ in $S$}
            \FOR {every sentence in $S_i$}
                \STATE Let $sp$ be the speaker in the sentence, $ts$ be the time stamp of the sentence.
                \IF {$sp \in M$}
                    \FOR {every $F_j$ exists in $ts$}
                    \STATE $\mathcal{C}_{L_j, sp} = \mathcal{C}_{L_j, sp} + 1$
                    \ENDFOR
                
                \ENDIF
            \ENDFOR
        \ENDFOR
        \FOR {every row in $\mathcal{C}$}
            \STATE Let $N_{max}$ be the largest number in the row, $N_{sec}$ be the second largest number in the row, $pc$ be the character name corresponds to $N_{max}$.
            \IF {$ N_{max}/N_{sec} > \theta$}
                \STATE Assign $pc$ to the group corresponding to the row.
            \ELSE
                \STATE Assign ``others" to the group corresponding to the row.
            \ENDIF
        \ENDFOR
  \RETURN face bounding boxes with assigned names
    \end{algorithmic}
\label{alg:naming}
\end{algorithm}

==> algorithm/pc_list.tex <==
\begin{algorithm}
    \caption{Determine Principal Character List}
    \begin{algorithmic}[1]
        \REQUIRE Subtitles $S = \{S_i\}$ in a TV show.
        \STATE Let $O$ be a blank set to store the occurrence for all speakers.
        \FOR {every $S_i$ in $S$}
            \FOR {every sentence in $S_i$}
                \STATE Let $sp$ be the speaker in the sentence.
                \IF {$sp \neq $ unknown \AND $sp \in O$ }
                    \STATE $O_{sp} = O_{sp} + 1$
                \ELSIF{$sp \neq $ unknown \AND $sp \not\in O$ }
                    \STATE $O_{sp} = 1$
                \ENDIF
            \ENDFOR
        \ENDFOR
        \STATE Let $M$ be a blank list to store principal characters.
        \FOR{every $sp$ in $O$}
            \IF{$O_{sp} > 500$}
               \STATE Add $sp$ to $M$.
            \ENDIF
        \ENDFOR
        \STATE Let $N_{max}$ be the highest of occurrence in $O$.
        \FOR{every $sp$ in $M$}
            \IF{$O_{sp} < N_{max}/10$}
               \STATE Remove $sp$ from $M$.
            \ENDIF
        \ENDFOR
  \RETURN the principal character list $M$
    \end{algorithmic}
\label{alg:pc_list}
\end{algorithm}

==> fig/case.tex <==
\begin{figure*}[thpb]
 \centering
 \includegraphics[height=7cm]{latex/images/case.png}
 \caption{Case study on the prediction results of our best model.}
\label{fig:case}
\end{figure*}

==> fig/character.tex <==
\begin{figure}[t!]
 \centering
 \includegraphics[height=6.2cm]{latex/images/actor-centric.png}
 \caption{In this work, we focus on character-centric relations. The three images with green borderlines are actor-centric relations, while the right-down image with red borderline is an example of character-unrelated relations.
}
\label{fig:character}
\end{figure}

==> fig/model_two_in_one.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.45\textwidth}
      \centering
      \includegraphics[width=0.9\textwidth]{latex/images/ICCV2019_model.pdf}
    \caption{Our Model}
    \label{fig:architecture}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.54\textwidth}
      \centering
      \includegraphics[width=\textwidth]{latex/images/ICCV2019_cooccurrence.pdf}
    \caption{Construction of the Co-occurrence Matrix}
    \label{fig:co-occurrence}
    \end{subfigure}
  \end{subfigure}
% \setlength\belowcaptionskip{-2ex}
\captionsetup{font=small}
\caption{(a) Architecture of our model. ``Q'' means the question and ``A0-A4'' are the 5 potential answers. ``Cross-Att'' is the cross attention module. The font colors of those visual features correspond to the colors of boxes in this frame. In practice we extract visual features from \textit{all} frames of an episode. The subtitles are from the episode that contains this frame. (b) The process of building the co-occurrence matrix between face clusters and characters' names. For each frame $t$, we increment the co-occurrence value of face $i$ and speaker $p$ if they appear together. Once the matrix is built, the face name of each row is obtained by the column that maximize the co-occurrence value.}
\label{fig:model}
\end{figure*}

% \begin{figure*}[t!]
%  \centering
%  \includegraphics[width=0.8\textwidth]{latex/images/ICCV2019_model.pdf}
%  \caption{Architecture of our model. ``Q'' means the question and ``A0-A4'' are the 5 potential answers. ``Cross-Att'' is the cross attention module. The font colors of those visual features correspond to the colors of boxes in this frame. In practice we extract visual features from \textit{all} frames of an episode. The subtitles are from the episode that contains this frame.}
% \label{fig:model}
% \end{figure*}

% \begin{figure*}[t!]
%  \centering
%  \includegraphics[height=7.8cm]{latex/images/ICCV2019_model.pdf}
%  \caption{Our multimodal temporal attentional transformer network.}
% \label{fig:model}
% \end{figure*}

==> fig/other_co.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}{\columnwidth}
    \centering
    \begin{subfigure}{0.49\columnwidth}
      \centering
      \includegraphics[width=0.9\textwidth]{latex/images/co-occurrence_friends.pdf}
    \caption{Friends}
    \label{fig:friends}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.49\columnwidth}
      \centering
      \includegraphics[width=0.95\textwidth]{latex/images/co-occurrence_grey.pdf}
    \caption{Grey}
    \label{fig:grey}
    \end{subfigure}
  \end{subfigure}
  \begin{subfigure}{\columnwidth}
    \centering
    \begin{subfigure}{0.49\columnwidth}
      \centering
      \includegraphics[width=0.95\textwidth]{latex/images/co-occurrence_house.pdf}
    \caption{House}
    \label{fig:house}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.49\columnwidth}
      \centering
      \includegraphics[width=0.88\textwidth]{latex/images/co-occurrence_castle.pdf}
    \caption{Castle}
    \label{fig:castle}
    \end{subfigure}
  \end{subfigure}
% \setlength\belowcaptionskip{-2ex}
\captionsetup{font=small}
\caption{Co-occurrence matrices of characters in other four TV shows (Friends, Grey, House, and Castle). The numbers in the matrices are presented in thousands.
% The brightness of tiles is proportional to their values. It is clear that each row of these matrices has a unique maximum value, whose column name is the corresponding character's name for the faces labeled with that row number.
``Others'' represent all the other supporting actors.}
\label{fig:other_co}
\end{figure}

==> fig/teaser.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}{\columnwidth}
    \centering
    \begin{subfigure}{0.85\columnwidth}
      \centering
      \includegraphics[width=\textwidth]{images/teaser_raj.jpeg}
    \end{subfigure}

    \centering
    \begin{subfigure}{0.85\columnwidth}
      \centering
      \includegraphics[width=\textwidth]{images/teaser_raj_qa.png}
    \end{subfigure}
  \end{subfigure}
\setlength\belowcaptionskip{-2ex}
\captionsetup{font=small}
\caption{Illustration of how fine-granular features may help in video story question answering. Character names, visual objects and their relationships are all necessary factors in answering this question.}
\label{fig:teaser}
\end{figure}

% \begin{figure}[t!]
%  \centering
%  \includegraphics[height=4.7cm]{latex/images/task.png}
%  \caption{A simple illustration of \textbf{Video Story Question Answering} task: given a video clip with subtitles and a multiple choice question about the contextual information, the goal is to correctly predict the right answer.}
% \label{fig:simple}
% \end{figure}

==> fig/three_co-occurrence_matrices.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.36\textwidth}
      \centering
      \includegraphics[width=0.9\textwidth]{latex/images/co-occurrence_bbt.pdf}
    \caption{BBT}
    \label{fig:bbt}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.315\textwidth}
      \centering
      \includegraphics[width=\textwidth]{latex/images/co-occurrence_met.pdf}
    \caption{HIMYM}
    \label{fig:met}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.315\textwidth}
      \centering
      \includegraphics[width=\textwidth]{latex/images/co-occurrence_friends.pdf}
    \caption{Friends}
    \label{fig:friends}
    \end{subfigure}
  \end{subfigure}
% \setlength\belowcaptionskip{-2ex}
\captionsetup{font=small}
\caption{Co-occurrence matrices of characters in BBT, HIMYM and Friends. The numbers in the matrices are presented in thousands. The brightness of tiles is proportional to their values. It is clear that each row of these matrices has a unique maximum value, whose column name is the corresponding character's name for the faces labeled with that row number. ``Others'' represent all the other supporting actors.}
\label{fig:three_co-occurrence}
\end{figure*}

==> fig/two_co-occurrence_matrices.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}{\columnwidth}
    \centering
    \begin{subfigure}{0.49\columnwidth}
      \centering
      \includegraphics[width=0.9\textwidth]{latex/images/co-occurrence_bbt.pdf}
    \caption{BBT}
    \label{fig:bbt}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.49\columnwidth}
      \centering
      \includegraphics[width=0.9\textwidth]{latex/images/co-occurrence_met.pdf}
    \caption{HIMYM}
    \label{fig:met}
    \end{subfigure}
  \end{subfigure}
% \setlength\belowcaptionskip{-2ex}
\captionsetup{font=small}
\caption{Co-occurrence matrices of characters in BBT and HIMYM. The numbers in the matrices are presented in thousands.
% The brightness of tiles is proportional to their values. It is clear that each row of these matrices has a unique maximum value, whose column name is the corresponding character's name for the faces labeled with that row number.
``Others'' represent all the other supporting actors.}
\label{fig:two_co-occurrence}
\end{figure}

==> fig/vrd_met.tex <==
\begin{figure}[t!]
 \centering
 \includegraphics[width=0.7\columnwidth]{latex/images/small-name-replace.png}
 \captionsetup{font=small}
 \caption{Examples of detected relations in \textit{HIMYM} video frames, where references to humans such as ``woman'' and ``man'' are replaced with predicted character names. Each human's name is determined by finding the face bounding box that overlaps the most with the human bounding box.
}
\label{fig:vrd_met}
\end{figure}

==> fig/vrd_model.tex <==
\begin{figure*}[thpb]
 \centering
 \includegraphics[height=7cm]{latex/images/relation.png}
 \caption{Overview of the adopted object and relation detection approach~\cite{zhang2018large}.}
\label{fig:relation}
\end{figure*}

==> tab/ablation_no_ts.tex <==
\begin{table}[t!]
\begin{center}
\begin{tabular}{clc}
\hline\noalign{\smallskip}   
Backbone & Method & Val\. Acc (w/o ts) \\ 
\noalign{\smallskip}
\toprule
\noalign{\smallskip}
\multirow{5}{*}{LSTM} & Sub & 66.14 \\
& Sub+Objs & 68.35 \\
& Sub+Objs\_nm & 68.43 \\
& Sub+Objs\_nm+Rels & 68.68 \\
& Sub+Objs\_nm+Rels\_nm & \textbf{68.90} \\
\noalign{\smallskip}
\bottomrule
\end{tabular}
\end{center}
\caption{Ablation study without time stamps on our modules. Abbreviations are the same with Table~\ref{tab:ablation_ts}.}
\label{tab:ablation_no_ts}
\end{table}

==> tab/action_ablation.tex <==
\begin{table}[t!]
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{lcc}
\hline\noalign{\smallskip}
 & \multicolumn{2}{c}{Val\. Acc} \\
Method & w/ ts & w/o ts \\ 
\noalign{\smallskip}
\toprule
\noalign{\smallskip}
Sub & 66.23 & 66.14 \\
Sub + Acts\_nm & 67.28 & 66.38 \\
Sub + Rels\_nm &  68.25  & 67.85\\
Sub + Rels\_nm + Acts\_nm & 68.18 & 67.42 \\
Sub + Objs\_nm & 69.45  & 68.13\\
Sub + Objs\_nm + Acts\_nm & 69.68 & 68.64 \\
Sub + Objs\_nm + Rels\_nm & 70.29 & 68.90\\
Sub + Objs\_nm + Rels\_nm + Acts\_nm & \textbf{70.50} & \textbf{69.12} \\
\noalign{\smallskip}
\bottomrule
\end{tabular}
}
\caption{Ablation study for adding action recognition results, both with and without the time stamps. ``Sub'', ``Objs'', ``Rels'', ``Acts'' and ``nm'' represent subtitles, objects, relationships, actions and names, respectively.}
\label{tab:ablation_act}
\end{table}

==> tab/actions.tex <==
\begin{table}
%\vspace{-5pt}
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular}
	{c} \hline
    catch, clap, climb, dive, drink, eat, fencing, golf, hit, \\
    hug, jump, kick, kiss, laugh, pick, pour, punch, push, \\
    ride, run, shake hands, shoot, sit, smile, smoke, stand, \\
    swing baseball, sword, talk, throw, turn, walk, wave \\\hline
\end{tabular}
\caption{The list of selected action classes.}
\label{tab:actions}
\end{table}

==> tab/qtype_ts.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.96\textwidth}{!}{
\begin{tabular}{lccccccc}
\hline\noalign{\smallskip}
 & \multicolumn{7}{c}{\textbf{Validation w/ ts}} \\
Method & what(55.62\%) & who(11.55\%) & where(11.67\%) & how(8.98\%) & why(10.38\%) & other(1.80\%) & all(100\%)\\ 
\noalign{\smallskip}
\toprule
\noalign{\smallskip}
Sub & 63.47 & 69.40 & 57.58 & 71.02 & 79.91 & 75.55 & 66.23 \\
Sub + Rels & 64.80 & 69.07 & 62.70 & 72.04 & \textbf{80.67} & 75.91 & 67.55  \\ 
Sub + Rels\_nm & 65.31 & 72.59 & 62.02 & 72.85 & 80.29 & 77.01 & 68.25  \\ 
Sub + Objs & 66.97 & 69.01 & 62.98 & 72.85 & 79.60 & 77.74 & 68.85 \\
Sub + Objs\_nm & 67.57 & 73.04 & 62.58 & 71.02 & 80.35 & \textbf{78.10} & 69.45  \\
Sub + Objs + Rels & 68.32 & 68.39 & 63.88 & 72.48 & 79.79 & 77.74 & 69.54 \\ 
Sub + Objs + Rels\_nm & 68.35 & 71.96 & 63.31 & \textbf{72.92} & 78.33 & 75.55 & 69.76  \\ 
Sub + Objs\_nm + Rels & 68.38 & \textbf{73.38} & 64.21 & 72.77 & 79.60 & \textbf{78.10} & 70.20  \\ 
Sub + Objs\_nm + Rels\_nm & \textbf{68.55} & 73.21 & \textbf{64.61} & 72.34 & 79.66 & 77.74 & \textbf{70.29}  \\
\noalign{\smallskip}
\bottomrule
\end{tabular}
}
\caption{The influence of question type for different methods with time stamps. ``Sub'', ``Objs'', ``Rels'' and ``nm'' represent subtitles, objects, relationships and names, respectively.}
\label{tab:qtype_ts}
\end{table*}

==> tab/stop_word.tex <==
\begin{table}
%\vspace{-5pt}
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular}
	{c} \hline
    `?', `,', `what', `who', `which', `is', `are', `the', `to', `of', \\ `there', `here', `a',
    `or', `and', `you', `any', `not', `see', \\`this', `that',  `have', `how', `has', `'s', 
    `either', `both', `as',\\ `was', `does', `do', `in', `on', `made', `make', `left', `right', \\
    `be', `behind', `same', `next', `near', `than', `photo', `image' \\\hline
\end{tabular}
\caption{The list of selected action classes.}
\label{tab:actions}
\end{table}
